Algebraic models of simple type theories: a polynomial approach

We develop algebraic models of simple type theories, laying out a framework that extends universal algebra to incorporate both algebraic sorting and variable binding. Examples of simple type theories include the unityped and simply-typed $\lambda$-calculi, the computational $\lambda$-calculus, and predicate logic. Simple type theories are given models in presheaf categories, with structure specified by algebras of polynomial endofunctors that correspond to natural deduction rules. Initial models, which we construct, abstractly describe the syntax of simple type theories. Taking substitution structure into consideration, we further provide sound and complete semantics in structured cartesian multicategories. This development generalises Lambek's correspondence between the simply-typed $\lambda$-calculus and cartesian-closed categories, to arbitrary simple type theories.

==> definitions.tex <==
\makeatletter
\newcommand{\xRightarrow}[2][]{\ext@arrow 0359\Rightarrowfill@{#1}{#2}}
\makeatother

\makeatletter
\newcommand{\xLeftarrow}[2][]{\ext@arrow 0359\Leftarrowfill@{#1}{#2}}
\makeatother

% Commands are often bracketed in {} to ensure they can be used sensible in sub/superscripts without explicit bracketing.

\newcommand{\cat}{\mathbf}
\newcommand{\defeq}{\stackrel{\textup{def}}{=}}
\newcommand{\Set}{\cat{Set}}
% \newcommand{\Top}{\cat{Top}}
\newcommand{\ptdSet}{\Set_{*}}
\newcommand{\Cat}{\cat{Cat}}
\newcommand{\CAT}{\cat{CAT}}
\newcommand{\FinSet}{\mathbb{F}}
\newcommand{\permset}{\mathbb{P}}
\newcommand{\comp}{\circ}
\newcommand{\vcomp}{\bullet}
\newcommand{\op}{^{\textup{op}}}
\newcommand{\too}{\longrightarrow}
\newcommand{\psh}{\widehat} % presheaf category
\newcommand{\spsh}[1]{\psh{\smcat{#1}}} % small presheaf
\newcommand{\Psh}[1]{\textup{Psh}(#1)}
\newcommand{\CoPsh}[1]{\textup{CoPsh}(#1)}
\newcommand{\pshF}{\psh{\finset}}
\newcommand{\adj}{\dashv}
\newcommand{\tuple}[1]{\langle#1\rangle}
\newcommand{\unit}{\tuple{}}
% Functor category
\newcommand{\fcat}[2]{[#1, #2]}
\newcommand{\inv}{^{-1}}
\newcommand{\id}[1]{\textup{id}_{#1}}
\newcommand{\Id}[1]{\textup{Id}_{#1}}
\newcommand{\alg}[1]{#1\textup{-}\cat{alg}}
\newcommand{\mon}[1]{\cat{#1\textup{-}mon}}
\newcommand{\ev}{\textup{ev}_}
\newcommand{\Lan}[2]{\textup{Lan}_{#1}(#2)}
\newcommand{\Ran}[2]{\textup{Ran}_{#1}(#2)}
\newcommand{\coend}[1]{\int^{#1}}
\newcommand{\isoto}{\xto{\cong}}
\newcommand{\natto}{\Rightarrow}
\newcommand{\xnatto}{\xRightarrow}
\newcommand{\natfrom}{\Leftarrow}
\newcommand{\xnatfrom}{\xLeftarrow}
\newcommand{\natiso}{\xnatto{\cong}}
\newcommand{\epito}{\twoheadrightarrow}
\newcommand{\epifrom}{\twoheadleftarrow}
\newcommand{\monoto}{\rightarrowtail}
\newcommand{\monofrom}{\leftarrowtail}
\newcommand{\codom}[1]{\textup{codom}(#1)}
\newcommand{\denote}[1]{{\llbracket #1 \rrbracket}}
\newcommand{\ob}[1]{|#1|} % object set of a category

\newcommand{\cata}{\mathscr{A}}
\newcommand{\catb}{\mathscr{B}}
\newcommand{\catc}{\mathscr{C}}
\newcommand{\catv}{\mathscr{V}}
\newcommand{\ct}{\mathscr}
\newcommand{\comma}{\downarrow}

\newcommand{\smcat}{\mathbb}
\newcommand{\sct}{\smcat}
\newcommand{\smcata}{\mathbb{A}}
\newcommand{\smcatb}{\mathbb{B}}
\newcommand{\initcat}{\mathbbm{0}}
\newcommand{\termcat}{\mathbbm{1}}

\newcommand{\nateq}{\simeq}
\newcommand{\injto}{\hookrightarrow}
\newcommand{\xto}{\xrightarrow}
\newcommand{\from}{\leftarrow}
\newcommand{\xfrom}{\xleftarrow}
\newcommand{\shlbox}[2]{\makebox[0pt][r]{\makebox[#1][l]{#2}}}
\newcommand{\xdownarrow}[3]{\text{\lapbox[\width]{2pt}{$\underset{#3}{\overset{#1}{\downarrow}}\text{\adjustbox{lap={\width}{-2pt}, raise=2pt}{$\scriptstyle #2$}}$}}}


\newcommand{\dom}{\textup{dom}}
\newcommand{\yonem}{\mathbf{y}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Hom}{\textup{Hom}}
% \newcommand{\st}{\enskip\vert\enskip}
\newcommand{\disc}[1]{\textup{disc}(#1)}
\newcommand{\el}[1]{\textup{el}(#1)}
\newcommand{\const}{\underline}
\newcommand{\diag}{\Delta}
\newcommand{\codiag}{\nabla}

\newcommand{\dsum}[1]{{\Sigma_{#1}}}
\newcommand{\pb}[1]{{#1^{*}}}
\newcommand{\dprod}[1]{{\Pi_{#1}}}
\newcommand{\precomp}[1]{{#1^{\star}}}
\newcommand{\kleene}{^{\star}}

\newcommand{\oper}{\mathsf}

% Typing rule
\newcommand{\tr}[2]{\trc{\Gamma}{#1}{#2}}
% Typing rule in extended context
\newcommand{\trec}[3]{\trc{\Gamma, #1}{#2}{#3}}
% Term with type
\newcommand{\twt}[2]{#1 : #2}
% Typing rule in context
\newcommand{\trc}[3]{#1 \vdash \twt{#2}{#3}}
% Typing rule in type context
\newcommand{\trtc}[3]{#1 \rhd \twt{#2}{#3}}
% Formation rule
\newcommand{\fr}[1]{#1\ \mathsf{type}}
% Formation rule in context
\newcommand{\frc}[1]{\Gamma \vdash \fr{#1}}

\newcommand{\subst}[3]{#1 [\sfrac{#2}{#3}]}

\let\jeq\equiv % judgemental equality
\renewcommand{\equiv}{\cong}
\let\smvec\vec
\renewcommand{\vec}{\overrightarrow}

\newcommand{\jneq}{\not\jeq}

\newcommand{\ssth}{\textsuperscript{th}}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{note}[theorem]{Note}
\newtheorem{remark}[theorem]{Remark}
% \newtheorem*{authornote}{Author's note}

\newcommand{\datetoday}{\date{\cleanlookdateon\today}}

\newcommand{\todo}[2][]{%
    \begin{mdframed}[backgroundcolor=red!20, hidealllines=true, #1]#2\end{mdframed}
}

\newcommand{\hr}{\vspace{20pt}\noindent\rule{\linewidth}{0.4pt}\vspace{20pt}}

% Latin abbreivations.
\newcommand{\latinabbr}{\emph}
\newcommand{\eg}{\latinabbr{e.g.}}
\newcommand{\ie}{\latinabbr{i.e.}}
\newcommand{\etc}{\latinabbr{etc.}}
\newcommand{\viz}{\latinabbr{viz.}}
\newcommand{\cf}{\latinabbr{cf.}}

\newcommand{\MLTT}{Martin-L\"of Type Theory}
\newcommand{\HoTT}{Homotopy Type Theory}
\newcommand{\lc}{\texorpdfstring{$\lambda$}{lambda}-calculus}
\newcommand{\lci}{\texorpdfstring{$\lambda$}{lambda}-calculi}
\newcommand{\stlc}{simply-typed \lc{}}
\newcommand{\Stlc}{Simply-typed \lc{}}
\newcommand{\ulc}{untyped \lc{}}
\newcommand{\Ulc}{Untyped \lc{}}
\newcommand{\llc}{linear \lc{}}
\newcommand{\Llc}{Linear \lc{}}
\newcommand{\plc}{polymorphic \lc{}}
\newcommand{\Plc}{Polymorphic \lc{}}
\newcommand{\clc}{computational \lc{}}
\newcommand{\CH}{Curry--Howard}
\newcommand{\CHL}{\CH{}--Lambek}
\newcommand{\CHc}{\CH{} correspondence}
\newcommand{\CHLc}{\CHL{} correspondence}
\newcommand{\gat}{generalised algebraic theory}
\newcommand{\gats}{generalised algebraic theories}
\newcommand{\Gats}{Generalised algebraic theories}
\newcommand{\eats}{essentially algebraic theories}
\newcommand{\Eats}{Essentially algebraic theories}
\newcommand{\nds}{natural deduction system}
\newcommand{\Nds}{Natural deduction system}
\newcommand{\noone}{no-one}

\newcommand{\sigty}[1][]{{\Sigma^{#1}_{\mathsf{ty}}}}
\newcommand{\sigtm}[1][]{{\Sigma^{#1}_{\mathsf{tm}}}}
\newcommand{\sigctx}[1][]{{\Sigma^{#1}_{\mathsf{ctx}}}}
\newcommand{\eqty}[1][]{{E^{#1}_{\mathsf{ty}}}}
\newcommand{\eqtm}[1][]{{E^{#1}_{\mathsf{tm}}}}
\newcommand{\eqctx}[1][]{{E^{#1}_{\mathsf{ctx}}}}

\newenvironment{sketch}{\renewcommand{\proofname}{Proof (sketch)}\proof}{\endproof}

\newcommand{\hy}{\text{-}}

\hyphenation{mono-sorted multi-sorted non-binding}
